Equitable Core Imputations for Max-Flow, MST and $b$-Matching Games

We study fair allocation of profit (or cost) for three central problems from combinatorial optimization: Max-Flow, MST and $b$-matching. The essentially unequivocal choice of solution concept for this purpose would be the core, because of its highly desirable properties. However, recent work [Vaz24] observed that for the assignment game, an arbitrary core imputation makes no fairness guarantee at the level of individual agents. To rectify this deficiency, special core imputations, called equitable core imputations, were defined - there are two such imputations, leximin and leximax - and efficient algorithms were given for finding them. For all three games, we start by giving examples to show that an arbitrary core imputation can be excessively unfair to certain agents. This led us to seek equitable core imputations for our three games as well. However, the ubiquitous tractable vs intractable schism separates the assignment game from our three games, making our task different from that of [Vaz24]. As is usual in the presence of intractability, we resorted to defining the Owen set for each game and algorithmically relating it to the set of optimal dual solutions of the underlying combinatorial problem. We then give polynomial time algorithms for finding equitable imputations in the Owen set. The motivation for this work is two-fold: the emergence of automated decision-making, with a special emphasis on fairness, and the plethora of industrial applications of our three games.

==> Arxiv/arXiv/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we explored the problem of finding fair and stable imputations in cooperative games, specifically focusing on the max-flow game, the min-cost branching game, and the $b$-matching game. Our primary objective was to investigate leximin/leximax fairness in the class of core imputations.


Even though for the assignment game, leximin and leximax core imputations can be computed in polynomial time due to the polynomial characterizability of the core, the situation is more complex for the games we considered. We proved the NP-hardness of finding a core imputation that maximizes the minimum profit or cost share for the max flow and min-cost branching games, thus ruling out the possibility of polynomial-time algorithms for computing leximin or leximax core imputations.

To address this intractability, we introduced an efficiently computable subclass of core, namely dual-consistent core (DCC) imputations. These are a subset of core imputations derived from solutions to the dual of the linear programs used to compute game values. For the max-flow game, and $b$-matching game we developed both LP-based and combinatorial algorithms to obtain leximin/leximax DCC imputations. For the min-cost branching game, we formulated the problem of finding the leximin/leximax DCC imputation using linear programs with exponentially many constraints and provided a separation oracle for the inequalities in these LPs. This demonstrated that the ellipsoid method could be used to obtain a polynomial-time algorithm for finding the leximin/leximax DCC imputation. Despite these advancements, we were unable to develop a combinatorial algorithm for finding the leximin/leximax DCC imputation for this game.

Our work highlights the potential of using dual LPs of games to identify a mathematically tractable subclass of core imputations. This approach can be particularly beneficial for games where the core is not easily characterized in polynomial time. Future research could further explore the properties of this subclass and examine its applicability in other types of games.

We propose two specific open questions related to the games we studied:
\begin{itemize}
\item Can an efficient combinatorial algorithm be developed for finding the leximin/leximax DCC in the min-cost branching game?
\item Is it NP-hard to test core membership in the $b$-matching game? If not, are there efficient algorithms for finding the leximin/leximax core imputation?
\end{itemize}

These questions underscore important avenues for future research, and addressing them will deepen our understanding of the combinatorial structures underlying the games we have studied.



% These questions highlight important directions for further investigation and would help deepen our understanding of equitable and stable imputations in cooperative games.
